How Diversely Can Language Models Solve Problems? Exploring the Algorithmic Diversity of Model-Generated Code

Language models (LMs) have exhibited impressive abilities in generating code from natural language requirements. In this work, we highlight the diversity of code generated by LMs as a critical criterion for evaluating their code generation capabilities. There is a lack of studies focused on assessing the diversity of generated code, which overlooks its importance in code LMs. Therefore, we propose a systematic approach to evaluate code diversity, introducing various metrics with inter-code similarity. Specifically, we introduce code clustering methods that leverages LMs' capabilities in code understanding and reasoning, resulting in a set of metrics that represent the number of algorithms in model-generated solutions. We extensively investigate the property of model-generated solutions by contrasting them with human-written ones and quantifying the impact of various factors on code diversity: model size, temperature, instruction tuning, and problem complexity. Our analysis demonstrates that model-generated solutions exhibit low algorithmic diversity, which was neglected by the research community. Moreover, we explore methods to increase code diversity by combining solutions from different models and increasing sampling temperatures. Our findings highlight that code diversity can be enhanced with the help of heterogeneous models and setting temperature beyond 1.0 that has not been fully explored due to the functional correctness degradation. To facilitate our research direction, we publicly share our code and datasets through open-source repositories.

==> legacy/041maintable.tex <==
\begin{table*}[h]
\centering
\small
% \resizebox{.99\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\textbf{Datasets} & \multicolumn{6}{c}{\textbf{\apps-Introductory}} & \multicolumn{6}{c}{\textbf{\apps-Interview}}  \\ 
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
Similarity measures & \multicolumn{2}{c}{\scc}  & \multicolumn{2}{c}{\codebert} & \multicolumn{2}{c}{\geval} &\multicolumn{2}{c}{\scc} &  \multicolumn{2}{c}{\codebert} & \multicolumn{2}{c}{\geval} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
Temperature ($\tau$) & 0.2 & 0.8 & 0.2 & 0.8 & 0.2 & 0.8  & 0.2 & 0.8 & 0.2 & 0.8 & 0.2 & 0.8 \\
\midrule
\codellamapython 7B & 14.0 & \ \ 2.0 & 71.9 & 48.7 & 42.5 & 13.8 & \ \ 8.0 & \ \ 2.8 & 71.6  & 52.1 & 32.5 & 10.5 \\
\codellamainstruct 7B & 52.0 & 27.6 & 89.7 & 81.8 & 65.7 & 53.5 & 50.4 & 14.4 & 92.1 & 80.2 & 60.4 & 42.3\\
\codellamapython 13B & 12.8 & \ \ 3.2 & 71.3 & 51.2 & 39.3 & 22.8 & 10.4 & \ \ 2.4 & 80.4 & 46.9 & 29.8 & 12.3\\

\codellamainstruct 13B & 52.0 & \underline{38.8} & 92.7 & 84.6 & 71.5 & \underline{59.8} & 40.0 & 18.4 & 91.5 & 84.3 & 59.6 & 45.3 \\
\codellamapython 34B & 2.0 & \ \ 1.2  & 46.4 & 46.3 & 14.6 & 14.2 & 1.2 & \ \ 0.4  & 38.8 & 50.0 & 8.9 & 8.1\\
\codellamainstruct 34B & 62.8 & \ \ 24.0  & \textbf{94.6} & 83.7 & 71.6 & 44.8 & \textbf{58.0} & \ \ \underline{20.8}  & \textbf{96.5} & \underline{87.2} & \textbf{70.6} & 41.8 \\
\starcoder 15B & 35.6 & \ \ 3.2 & 80.3 & 52.1 & 49.8 & 22.3 & 14.4 & \ \ 4.8 & 81.7  & 54.8 & 44.8 & 16.9\\
\starcoderinstruct 15B &47.6 & 18.4 & 86.7 & 73.8 & 69.2 & 51.2 & 45.2 & \ \ 3.6 & 84.2 & 62.2 & 57.8 & 29.8 \\
\deepseek 6.7B & 24.4 & \ \ 2.4 & 74.9 & 57.6 & 42.3 & 21.7 & 14.4 
 & \ \ 2.4 & 70.2 & 52.7 & 27.8 & \ \ 9.5 \\
\deepseekinstruct 6.7B & 50.0 & 15.6 & 84.9 & 74.3 & 64.5 & 43.5 & 28.4 & 10.8 & 81.7 & 66.6 & 46.5 & 28.8 \\
\gptturbo & \textbf{65.2}  & 37.6  & 94.4 & \underline{89.1} & \textbf{76.8} & 43.2 & 40.4  & 19.6 & 93.9 & 83.6 & 56.8 & \underline{48.1} \\
\midrule

\textbf{Datasets} & \multicolumn{6}{c}{\textbf{\apps-Competition}} & \multicolumn{6}{c}{\textbf{\humaneval}} \\ \cmidrule(lr){2-7} \cmidrule(lr){8-13}
Similarity measures & \multicolumn{2}{c}{\scc} & \multicolumn{2}{c}{\codebert} & \multicolumn{2}{c}{\geval} &\multicolumn{2}{c}{\scc} &  \multicolumn{2}{c}{\codebert} & \multicolumn{2}{c}{\geval} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
Temperature ($\tau$) & 0.2 & 0.8 & 0.2 & 0.8 & 0.2 & 0.8 & 0.2 & 0.8 & 0.2 & 0.8 & 0.2 & 0.8 \\ 
\midrule
\codellamapython 7B & \ \ 5.6 & \ \ 1.6 & 71.2 & 43.8 & 28.3 & \ \ 7.2 & 80.5 & 12.7 & 97.1 & 94.0 & 75.0 & 31.8 \\
\codellamainstruct 7B & 28.8 & \ \ 6.8 & 91.0 & 76.4 & 50.1 & 31.5 & \textbf{97.7} & 61.4 & \textbf{99.9} & 98.0 & \textbf{96.0} & 72.5 \\
\codellamapython 13B & \ \ 9.6 & \ \ 1.6 & 79.6 & 45.1 & 21.5 & \ \ 9.1 & 85.8 & 15.2 & 98.7 & 94.3 & 81.8 & 48.9 \\
\codellamainstruct 13B &  30.8 & 12.8 & 90.8 & 83.8 & 56.8 & 32.1 & \textbf{97.7} & \underline{65.4} & 99.4 & \underline{98.1} & 93.8 & \underline{82.3} \\
\codellamapython 34B & 12.0 & \ \ 0.8  & 70.8 & 44.6 & 27.8 & 6.5 & 47.2 & \ \ 9.2  & 95.3 &  81.7& 74.1 & 42.8 \\
\codellamainstruct 34B & \textbf{48.4} & \ \ \underline{17.6}  & \textbf{93.3} & \underline{85.1} & \textbf{62.5} & 33.5 & 81.6 & \ \ 61.2 & 99.0 & \underline{98.1} & 91.8 & 72.6\\
\starcoder 15B & \ \ 6.4 & \ \ 2.0 & 75.6 & 50.2 & 32.6 & 11.5 & 77.5 & \ \ 7.7 & 96.5 & 93.4 & 76.5 & 42.3 \\
\starcoderinstruct 15B & 33.6 & \ \ 2.4 & 80.4 & 55.5 & 48.3 & 25.5 & 81.3& 34.1 & \textbf{99.9}  & 95.5  & 85.3 & 65.8 \\
\deepseek 6.7B & \ \ 1.2 & \ \ 1.2 & 45.2 & 46.5 & \ \ 8.5 & \ \ 6.8 & 80.4 & 10.6 & 97.4 & 93.5 & 79.3 & 49.5 \\
\deepseekinstruct 6.7B & 31.6 & \ \ 7.2 & 81.5 & 64.8 & 41.5 & 23.8 & 95.5 & 34.1 & 99.9 & 96.5 & 84.3 & 63.5 \\
\gptturbo & 31.6 & 12.0 & 91.3 & 83.2 & 49.6 & \underline{40.1} & 70.8 & 61.2 & 97.2 & 95.3 & 81.2 & 77.3 \\
\bottomrule
\end{tabular}
% }
\caption{Similarity of codes (\%) generated by various sizes of code LMs based on three evaluation methods: \scc, CodeBERT, and LLM-Eval. 
For each (dataset, metric) pair, the highest similarity scores are highlighted in bold for those generated with a temperature of 0.2, and underlined for those generated with a temperature of 0.8.}
\label{tbl:maintable}
\end{table*}
